LISSNAS: Locality-based Iterative Search Space Shrinkage for Neural Architecture Search

Search spaces hallmark the advancement of Neural Architecture Search (NAS). Large and complex search spaces with versatile building operators and structures provide more opportunities to brew promising architectures, yet pose severe challenges on efficient exploration and exploitation. Subsequently, several search space shrinkage methods optimize by selecting a single sub-region that contains some well-performing networks. Small performance and efficiency gains are observed with these methods but such techniques leave room for significantly improved search performance and are ineffective at retaining architectural diversity. We propose LISSNAS, an automated algorithm that shrinks a large space into a diverse, small search space with SOTA search performance. Our approach leverages locality, the relationship between structural and performance similarity, to efficiently extract many pockets of well-performing networks. We showcase our method on an array of search spaces spanning various sizes and datasets. We accentuate the effectiveness of our shrunk spaces when used in one-shot search by achieving the best Top-1 accuracy in two different search spaces. Our method achieves a SOTA Top-1 accuracy of 77.6\% in ImageNet under mobile constraints, best-in-class Kendal-Tau, architectural diversity, and search space size.

==> abstract_backup.tex <==
Search spaces hallmark the advancement of Neural Architecture Search (NAS) methods. Despite many contributions to NAS research, large search spaces still present challenges with performance and search efficiency. Search spaces with large cardinality are less efficient and are associated with a higher likelihood of suboptimal search: accurate modeling of the space proves challenging. 

Alternatively, search space shrinkage methods have been proposed for selecting a region (within the space) with a higher density of well-performing networks. % do we need to say this next line?, commenting out for now% 
%Typically, these algorithms prune architectures with certain operations to shrink the search space. %%
Although small performance and efficiency gains are observed by incorporating these methods, such techniques prune some well-performing architectures in regions of the search space with lower densities of well-performing networks. As a result, current shrinkage algorithms are ineffective at retaining the \emph{granularity} of the original search space: the diversity and proportion of well-performing architectures. 

Our algorithm, LISSNAS, generates a granular, shrunk search space by leveraging locality - the property that structural similarity correlates to performance similarity. We showcase our approach on 4 different search spaces in 6 different datasets and extensively evaluate the properties of our shrunk search spaces. Compared to existing approaches, our search space increases the proportion of well-performing networks, improves performance during search, and runs more efficiently. Additionally, while the output of LISSNAS can be used for any NAS search method, we demonstrate its effectiveness in one-shot search. LISSNAS achieves a SOTA Top-1 accuracy of {XXX} in ImageNet under mobile constraints, best-in-class Kendal-Tau of {XXX}, network diversity, and search space size. 
